Scalable Approximate Inference and Some Applications

Approximate inference in probability models is a fundamental task in machine learning. Approximate inference provides powerful tools to Bayesian reasoning, decision making, and Bayesian deep learning. The main goal is to estimate the expectation of interested functions w.r.t. a target distribution. When it comes to high dimensional probability models and large datasets, efficient approximate inference becomes critically important. In this thesis, we propose a new framework for approximate inference, which combines the advantages of these three frameworks and overcomes their limitations. Our proposed four algorithms are motivated by the recent computational progress of Stein's method. Our proposed algorithms are applied to continuous and discrete distributions under the setting when the gradient information of the target distribution is available or unavailable. Theoretical analysis is provided to prove the convergence of our proposed algorithms. Our adaptive IS algorithm iteratively improves the importance proposal by functionally decreasing the KL divergence between the updated proposal and the target. When the gradient of the target is unavailable, our proposed sampling algorithm leverages the gradient of a surrogate model and corrects induced bias with importance weights, which significantly outperforms other gradient-free sampling algorithms. In addition, our theoretical results enable us to perform the goodness-of-fit test on discrete distributions. At the end of the thesis, we propose an importance-weighted method to efficiently aggregate local models in distributed learning with one-shot communication. Results on simulated and real datasets indicate the statistical efficiency and wide applicability of our algorithm.

==> tex/conclusion.tex <==
\section{CONCLUSION}
In this paper, we propose an efficient algorithm for sampling from discrete distributions based on gradient-free SVGD. We demonstrate the effectiveness of our algorithm on a number of discrete graphical models. Leveraging our method, we propose a new promising approach for  training  ensembles of binarized neural networks.  
Future research includes applying our ensemble method to training BNN with  larger networks such as VGG net and  larger dataset such as ImageNet dataset. 

% In future work, we would like to be devoted to extend this framework to both large scale real-world dataset and large scale discrete models, such as binarized Resnet or binarized LSTM. Furthermore,, to combine our framework with several recently proposed relax method such as Gumble-softmax is also an exciting work. In particular, designing more energy-efficient and hardware-friendly architecture is a promising direction toward applications on mobile devices.

==> tex/gf_introduction.tex <==
\section{Introduction}
\renewcommand{\F}{\mathcal{F}}
Approximate inference of complex distributions is a long-standing fundamental computational task in machine learning and statistics. 
Traditional methods are based on either Markov chain Monte Carlo (MCMC) \citep{neal2011mcmc, hoffman2014no}, or variational inference (VI) \citep{blei2017variational, zhang2017advances}, both of which have their own inherent pros and cons: MCMC is theoretically sound and asymptotically consistent, but is often slow to converge in  practice; VI is practically faster but has been known to lack theoretical consistency guarantees. 

Stein variational gradient descent (SVGD) \citep{liu2016stein} is recently developed to integrate the advantages of MCMC and VI. 
By leveraging a new type of functional gradient descent of KL divergence on the space of distributions, 
SVGD directly fits a set of non-parametric particles to the distribution of interest, without introducing additional parametric forms. This makes SVGD both theoretically sound \citep{liu2017stein}, practically fast and sample-efficient thanks to its optimization-based formulation. 

Unfortunately, gradient information of the target distribution is not always available in practice. 
In some cases, the distribution of interest is only available as a black-box density function and the gradient cannot be calculated analytically; in other cases, it may be computationally too expensive to calculate the gradient \citep{beaumont2003estimation, andrieu2009pseudo, filippone2014pseudo}. The goal of this paper is to extend SVGD to gradient-free settings. 

\textbf{Our Results}~ 
We propose a simple gradient-free variant of SVGD that replaces the true gradient with a surrogate gradient and uses a form of importance weighting to correct the bias introduced by the surrogate gradient.  
To give a very quick overview of our method, recall that the standard SVGD 
approximates a given distribution $p$ on $\R^d$ with a set of particles $\{\vx_i\}_{i=1}^n$ iteratively updated by 
$\vx_i \gets \vx_i  + \frac{\epsilon}{n} \Delta \vx_i$, where 
\begin{align}\label{update11}
\!\!\!\!\! \Delta \vx_i =\sum_{j=1}^n [\nabla \log p(\vx_j)k(\vx_j, \vx_i) +  \nabla_{\vx_j}k(\vx_j,\vx_i)], 
\end{align}
where $k(\vx,\vx')$ is any positive definite kernel; the term with gradient $\nabla\log p$ drives the particles to the high probability regions of $p$,
and the term with $\nabla k(\vx, \vx')$ acts as a repulsive force to keep the particles away from each other to quantify the uncertainty. 

\newcommand{\scalemath}[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}
Our gradient-free SVGD is based on the following generalization of the SVGD update rule: % \eqref{update11} to a more general update rule: 
\begin{align}
\scalemath{0.99}{
%\resizebox{1\hsize}{!}{
\label{update222}
\!\!\!\!\!\! \Delta \vx_i \propto
%\frac{\epsilon_i}{Z}\frac{\epsilon}{n}
\!\sum_{j=1}^n 
\!w_j \big[\nabla \log \rho(\vx_j) k( \vx_j, \vx_i) + \nabla_{\vx_j} k(\vx_j, \vx_i) \big], 
}
\end{align}
which replaces the true gradient $\nabla \log p$ with a surrogate gradient $\nabla\log \rho$ of an arbitrary auxiliary distribution $\rho(\vx)$, and then uses an importance weight $w_j:=\rho(\vx_j)/p(\vx_j)$ to correct the bias introduced by the surrogate.
Perhaps surprisingly, 
we show that the new update can be derived as a standard SVGD update by using an importance weighted kernel $w(\vx)w(\vx')k(\vx,\vx')$, and hence immediately inherits the theoretical proprieties of SVGD; 
for example, particles updated by \eqref{update222} can be viewed as a gradient flow of KL divergence similar to the original SVGD \citep{liu2017stein}. 

The performance of the gradient-free update \eqref{update222} critically depends on the choice of $\rho$. We study this problem empirically and show that it works efficiently, sometimes even better than the original SVGD, if we take $\rho$ to be an \emph{over-dispersed} estimate of $p$ that covers the support of $p$ well. We further improve the algorithm by combining the gradient-free update \eqref{update222} with simulated annealing, which we show consistently outperforms 
a number of other advanced gradient-free Monte Carlo methods, including a gradient-free variant of annealed importance sampling \citep{neal2001annealed}, kernel adaptive Metropolis-Hastings (KAMH) \citep{sejdinovic2014kernel} and kernel  Hamiltonian  Monte Carlo  (KHMC) \citep{strathmann2015gradient}. 

\paragraph{Related Works on Discrete Distribution Sampling} 
Almost all gradient-free sampling methods employ some auxiliary (or proposal) distributions that are different, but sufficiently close to the target distribution, followed with some mechanisms to correct the bias introduced by the surrogate distribution. 
There have been a few number of bias-correction mechanisms underlying most of the gradient-free methods, 
including importance sampling, rejection sampling and the Metropolis-Hastings rejection trick. 
The state-of-the-art gradient-free sampling methods are often based on adaptive improvement of the proposals  
when using these tricks, this includes adaptive importance sampling and rejection sampling \citep[]{gilks1992adaptive, cappe2008adaptive, cotter2015parallel, han2017stein}, and adaptive MCMC methods \citep[e.g.,][]{sejdinovic2014kernel, strathmann2015gradient}.  
 
Our method is significantly different from these gradient-free sampling algorithms aforementioned in principle, with a number of key advantages. 
Instead of correcting the bias by either re-weighting or rejecting the samples from the proposal, which unavoidably reduces the effective number of usable particles,  
our method re-weights the SVGD gradient and steers the update direction of the particles in a way that compensates the discrepancy between the target and surrogate distribution, without directly reducing the effective number of usable particles. 

In addition, 
while the traditional importance sampling and rejection sampling methods require the proposals to be simple enough to draw samples from, 
our update does not require to draw samples from the surrogate $\rho$. We can set $\rho$ to be arbitrarily complex as long as we can calculate  $\rho(\vx)$ and its gradient.  
In fact, $\rho(\vx)$ does not even have to be a normalized probability, sidestepping the difficult problem of calculating the normalization constant.  

{\bf Outline} The paper is organized as follows. 
Section 2 introduces the background of SVGD. 
Section~3 introduces our novel gradient-free SVGD algorithm, and Section~4 further proposes annealed gradient-free SVGD that combines the advantage of simulated annealing to achieve better performance for complex distributions. 
We present empirical results in Section~5 and conclude the paper in Section~6. 

